Massive runaways and walkaway stars

Anticipating the kinematic constraints from the Gaia mission, we perform an extensive numerical study of the evolution of massive binary systems to predict the peculiar velocities that stars obtain when their companion collapses and disrupts the system. Our aim is to (1) identify which predictions are robust against model uncertainties and assess their implications, (2) investigate which physical processes leave a clear imprint and may therefore be constrained observationally and (3) provide a suite of publicly available model predictions. We find that $22_{-8}^{+26}$% of all massive binary systems merge prior to the first core collapse in the system. Of the remainder, $86_{-9}^{+11}$% become unbound because of the core-collapse. Remarkably, this rarely produce runaway stars (i.e., stars with velocities above 30 km/s). These are outnumbered by more than an order of magnitude by slower unbound companions, or "walkaway stars". This is a robust outcome of our simulations and is due to the reversal of the mass ratio prior to the explosion and widening of the orbit, as we show analytically and numerically. We estimate a $10^{+5}_{-8}$% of massive stars to be walkaways and only $0.5^{+1.0}_{-0.4}$% to be runaways, nearly all of which have accreted mass from their companion. Our findings are consistent with earlier studies, however the low runaway fraction we find is in tension with observed fractions 10%. If Gaia confirms these high fractions of massive runaway stars resulting from binaries, it would imply that we are currently missing physics in the binary models. Finally, we show that high end of the mass distributions of runaway stars is very sensitive to the assumed black hole natal kicks and propose this as a potentially stringent test for the explosion mechanism. We discuss companions remaining bound which can evolve into X-ray and gravitational wave sources.

==> figures/fig_tree/tree.tex <==
%% requires:
% \usepackage{tikz-qtree}
% \usetikzlibrary{shadows,trees}


\tikzset{font=\small,
edge from parent fork down,
level distance=2cm,
sibling distance=3pt,
every node/.style={top color=blue!15,
  bottom color=blue!15,
  rectangle,rounded corners,
  minimum height=0mm,
  % draw=blue!75,
  % very thick,
  % drop shadow,
  align=center,
  % text depth = 0pt
},
% level 0/.style={level distance=2cm},
% level 1/.style={level distance=1.3cm},
% level 2/.style={sibling distance=-50pt},
% level 3/.style={sibling distance=-20pt},
level 4/.style={sibling distance=20pt},
level 5/.style={sibling distance=10pt},
edge from parent/.style={
  draw=blue!50,
  very thick,
},
blank/.style={draw=none},
}

\begin{tikzpicture}
  \Tree [
          .{Binaries with\\$M_1^\mathrm{ZAMS}\geq7.5\,M_\odot$\\ $q^\mathrm{ZAMS}\geq0.1$\\$0.15\leq \log_{10}(P^\mathrm{ZAMS}/\mathrm{days})\leq 5.5$}
               \edge [] node [draw=none, top color=white, bottom
               color=white, above, xshift=-10pt] {$22_{-9}^{+26}\%$};
               [
                   .{Stellar\\mergers}
               ]
               \edge [] node [draw=none, top color=white, bottom
               color=white, above, xshift=10pt] {$78_{-22}^{+9}\%$};
               [
                   .{Non mergers}
                   \edge [] node [draw=none, top color=white, bottom color=white, midway, above] {$1-\mathcal{D}=14_{-10}^{+22}\%$};
                   [
                       .{Non Disrupted\\ {\tiny
                           (cf.~\Secref{sec:bound})}}
                                          \edge [] node [draw=none, top color=white, bottom color=white, midway, left] {$36_{-15}^{+42}\%$};
                       [
                       .{NS companion}
                       ]
                       \edge [] node [draw=none, top color=white, bottom color=white, midway, right] {$64_{-42}^{+15}\%$};
                       [
                       .{BH companion}
                       ]
                   ]                       
                   \edge [] node [draw=none, top color=white, bottom color=white, midway, above] {\textcolor{red}{$\mathcal{D}=86_{-22}^{+10}\%$}};
                   [
                       .{Disrupted}
                       \edge [] node [draw=none, top color=white, bottom color=white, midway, above] {$25_{-10}^{+8}\%$};
                       [
                           .{post-MS companion \\ {\tiny
                               (cf.~\Secref{sec:non-MS-companions})}}
                           \edge [] node [draw=none, top color=white,
                           bottom color=white,  above, xshift=-6pt] {$53_{-46}^{+12}\%$};
                           [
                              .{WD}
                           ]
                           \edge [] node [draw=none, top color=white,
                           bottom color=white,
                           below, yshift=-40pt] {$23_{-20}^{+38}\%$};
                           [
                               .{He star}
                           ]
                           \edge [] node [draw=none, top color=white,
                           bottom color=white,  above, xshift=6pt] {$25_{-6}^{+23}\%$};
                           [
                               .{H-rich}
                           ]                        
                      ]
                      \edge [] node [draw=none, top color=white, bottom color=white, midway, above] {$75_{-8}^{+10}\%$};
                      [
                           .{MS companion \\ {\tiny (cf.~\Secref{sec:MS})}}
                           \edge [] node [draw=none, top color=white,
                           bottom color=white, above, xshift=-3pt] {$5_{-2}^{+14}\%$};
                           [
                              .{Runaway\\$v_\mathrm{dis}\geq30\,\mathrm{km\ s^{-1}}$}
                           ]
                           \edge [] node [draw=none, top color=white,
                           bottom color=white, above, xshift=+3pt] {$95_{-14}^{+2}\%$};
                           [
                               .{Walkaway\\$v_\mathrm{dis}<30\,\mathrm{km\ s^{-1}}$}
                           ]                              
                     ]
                   ]       
               ]
        ]    
\end{tikzpicture}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../walkaway"
%%% End:

